Unraveling Attacks in Machine Learning-based IoT Ecosystems: A Survey and the Open Libraries Behind Them

The advent of the Internet of Things (IoT) has brought forth an era of unprecedented connectivity, with an estimated 80 billion smart devices expected to be in operation by the end of 2025. These devices facilitate a multitude of smart applications, enhancing the quality of life and efficiency across various domains. Machine Learning (ML) serves as a crucial technology, not only for analyzing IoT-generated data but also for diverse applications within the IoT ecosystem. For instance, ML finds utility in IoT device recognition, anomaly detection, and even in uncovering malicious activities. This paper embarks on a comprehensive exploration of the security threats arising from ML's integration into various facets of IoT, spanning various attack types including membership inference, adversarial evasion, reconstruction, property inference, model extraction, and poisoning attacks. Unlike previous studies, our work offers a holistic perspective, categorizing threats based on criteria such as adversary models, attack targets, and key security attributes (confidentiality, availability, and integrity). We delve into the underlying techniques of ML attacks in IoT environment, providing a critical evaluation of their mechanisms and impacts. Furthermore, our research thoroughly assesses 65 libraries, both author-contributed and third-party, evaluating their role in safeguarding model and data privacy. We emphasize the availability and usability of these libraries, aiming to arm the community with the necessary tools to bolster their defenses against the evolving threat landscape. Through our comprehensive review and analysis, this paper seeks to contribute to the ongoing discourse on ML-based IoT security, offering valuable insights and practical solutions to secure ML models and data in the rapidly expanding field of artificial intelligence in IoT.

==> tex/introduction/attack_classification.tex <==
In this section, we classify six attack methods from three dimensions: black box attack and white box attack, active attack and passive attack, data attack and model attack, and give corresponding definitions.
%black/white-box
\begin{itemize}
    \item Adversary Knowledge: White-Box Attacks and Black-Box Attacks are two attack models in the field of machine learning. They describe the difference in the attacker's understanding of the target machine learning model.
\end{itemize}

（1）White-box Attacks: A white-box attack\cite{biryukov2018attacks} occurs when the attacker has detailed knowledge of the target model, including the model’s internal structure, parameters, weights, and training data. An attacker may have all the information about the model.
%In a white-box attack, the attacker can directly analyze the inner workings of the target model and precisely design an attack strategy to exploit the model's weaknesses or vulnerabilities.\\
White-box attacks are often easier to implement because the attacker can leverage deep knowledge of the target model to discover vulnerabilities in the model.

（2）Black-box Attacks: A black box attack\cite{bhagoji2018practical} means that the attacker can only access the input and output of the target model but knows nothing about the model's internal structure, parameters, and weights. The attacker does not have access to the details of the target model.
%In a black-box attack, the attacker attempts to infer the model's sensitive information, confidentiality, or internal structure from external characteristics of the target model, such as the model's prediction results.\\
Black-box attacks are generally more challenging because the attacker needs to reverse engineer the behavior of the target model through experimentation and observation without being able to see its internals directly.


%activate/passive attacks
%\begin{itemize}
%\item Adversary Behavior: In the field of machine learning and cybersecurity, active attacks and passive attacks are two different types of attacks that operate against the security and privacy of a system or model.
%\end{itemize}

%（1）Active Attacks: An active attack is when an attacker takes active actions to intentionally disrupt, corrupt, or modify machine learning models or training data to achieve their malicious goals.

%（2）Passive Attacks: A passive attack is when an attacker observes, listens, or collects information without modifying or interfering with the machine learning model or training data. In passive aggression, the attacker's primary goal is to obtain sensitive information or understand the model's behavior without causing apparent interference.
%data/model attacks

\begin{itemize}
    \item Adversary Ability: When it comes to machine learning security, we need to consider two main types of attacks: Data Attacks and Model Attacks. These attacks can threaten machine learning models' performance, privacy, and security.
\end{itemize}

（1）Data Attacks: In a data attack, an attacker attempts to affect the performance or output of a machine learning model by modifying, tampering, or manipulating training data or input data.
%The goal of data attacks is usually to trick the model or cause the model to produce incorrect predictions. For example, an attacker can add noise to training data, falsify data points, delete or modify data examples to cause the model to make incorrect decisions when faced with similar data.

（2）Model Attacks:  In a model attack, an attacker attempts to obtain or abuse the machine learning model's information, parameters, weights, structure, or output for improper purposes.
%Model attacks often target model confidentiality, intellectual property, or the privacy of model outputs. For example, an attacker might attempt to perform model reverse engineering to reconstruct the model's internal structure or parameters. This can be called a model extraction attack.\\


\begin{figure}[!ht]
     \centering
     \includegraphics[width=1.0\linewidth]{Picture/overview.pdf}
     \caption{Overview of Machine learning attacks. We classify machine learning attacks from two dimensions. First, we divide the attacks into active and passive attacks and list the specific attack methods. Secondly, we classify machine learning attacks in sequence according to three security factors: confidentiality, integrity, and availability.}
     \label{Fig}
\end{figure}

\begin{table}[!ht]
     \renewcommand{\tablename}{Table}
     \centering
     \includegraphics[width=1.0\linewidth]{Table/drawio.pdf}
     \caption{Overview of Attacking methods for each attack type. We classify the six attacks based on the six dimensions of Learning: GAN, Gradient-based, Shadow Training, Threshold, and Equation-solving, as shown in Table 1. We focus on explaining that Learning technology uses model parameters and gradients as inputs to the classifier or input and output queries to create alternative models.}
     \label{Fig8}
\end{table}

\begin{figure}[!ht]
     \centering
     \includegraphics[width=0.6\linewidth]{Picture/Library.pdf}
     \caption{Overview of the library for each attack type. We count the number of six types of attacks based on the number of libraries we reference in the article. MIA is represented by Membership inference attacks, AA is represented by Adversarial attacks, Ra is represented by Reconstruction attacks, PIA is represented by property inference attacks, and Model extraction attacks represent MEA, PA is represented as Poisoning attacks. Original Library means that the paper was implemented by the author, Unoriginal Library means a library provided by other individuals or entities, and N/A means that we cannot determine whether the library is open sourced by the author of the paper.}
     \label{Fig9}
\end{figure}

==> tex/introduction/secure_challenges.tex <==
As we enter the world of ML-based IoT, we are greeted with endless possibilities but also faced with significant security challenges. ML-based IoT is a powerful technology that allows computers to learn from data and make automated decisions. However, this ability makes ML-based IoT systems a potential target for attackers and can lead to a wide range of security risks.
In the previous section, we discussed the security risks ML-based IoT poses. Next, we'll explore these security challenges posed by ML-based IoT and understand how they impact our society and technological applications. At the same time, we will also explore methods and solutions to address these challenges to ensure that the development of ML-based IoT can occur in a safe and trusted environment. In this field of challenges and opportunities, it is crucial to understand security issues to ensure that the future of ML-based IoT is positive, innovative, and secure.

\subsubsection{Privacy Issues}
ML-based IoT models require large amounts of data during training and inference, including personal, sensitive, or commercially confidential information. Disclosure of this data could result in serious privacy violations.

\subsubsection{Model Protection}
ML-based IoT models themselves can become targets of attacks. Attackers may attempt to obtain model parameters, architecture, or knowledge, resulting in intellectual property infringement, model misappropriation, or improper use.

\subsubsection{Data Injection and Tampering}
Attackers can deliberately inject malicious data or tamper with training data to affect the model's performance. This poisoning attack can cause the model to produce incorrect predictions.

\subsubsection{Model Bias and Unfairness}
ML-based IoT models learn social or data biases in the training data, which may lead to unfair decisions.

\subsubsection{Interpretability and Transparency}
Deep learning models are often viewed as black boxes, making it challenging to explain their decision-making processes. This can lead to difficulties and uncertainty in applications that require interpretability.

